Low-rank Matrix Completion using Alternating Minimization

Alternating minimization represents a widely applicable and empirically successful approach for finding low-rank matrices that best fit the given data. For example, for the problem of low-rank matrix completion, this method is believed to be one of the most accurate and efficient, and formed a major component of the winning entry in the Netflix Challenge. In the alternating minimization approach, the low-rank target matrix is written in a bi-linear form, i.e. $X = UV^\dag$; the algorithm then alternates between finding the best $U$ and the best $V$. Typically, each alternating step in isolation is convex and tractable. However the overall problem becomes non-convex and there has been almost no theoretical understanding of when this approach yields a good result. In this paper we present first theoretical analysis of the performance of alternating minimization for matrix completion, and the related problem of matrix sensing. For both these problems, celebrated recent results have shown that they become well-posed and tractable once certain (now standard) conditions are imposed on the problem. We show that alternating minimization also succeeds under similar conditions. Moreover, compared to existing results, our paper shows that alternating minimization guarantees faster (in particular, geometric) convergence to the true matrix, while allowing a simpler analysis.

==> conclusion.tex <==
\section{Conclusion}

==> sensing-noisycase.tex <==
\subsection{Noisy Case}
\label{sec:sensing_noisycase}
We now consider an extension of the matrix sensing problem where measurements can be corrupted arbitrarily using a bounded noise. That is, we 
%We now extend Theorem \ref{thm:sensing} in the presence of noise. In particular, we consider the case where we 
observe $b=\aff\left(M+N\right)$, where $N$ is the noise matrix. % s.t.,
%\begin{align}\label{eqn:matrix-noisy}
%  M = U^* \Sigma^* {V^*}^{\dag},\ \ \ 
%  N = \Un \Sn (\Vn)^{\dag},
%\end{align}
%nd $N=\Un \Sn (\Vn)^{\dag}$ is the SVD of the noise matrix $N$. 
For this noisy case as well, we show that \as recovers $M$ upto an additive approximation depending on the Frobenius norm of  $N$. 
\begin{theorem}\label{thm:sensing-noisycase}
 Let $M$ and $\calA(\cdot)$ be as defined in Theorem~\ref{thm:sensing_err}. Suppose, \as algorithm (Algorithm \ref{algo:sensing-altmin}) is supplied inputs $\aff$, $b=\aff(M+N)$, where $N$ is the noise matrix s.t. $\left\|N\right\|_F  < \frac{1}{100}\so_k$.  Then, after $T=4\log(2/\epsilon)$ steps, iterates $\widehat{U}^{T}$, $\widehat{V}^{T}$ of \as  satisfy: 
%   Let $M=U^*\Sigma^*V^{*^\dag }$ be a rank-$k$ matrix with non zero singular values $\sigma_1^*\geq \sigma_2^*\dots\geq \sigma_k^*$ and $N=\Un \Sn (\Vn)^{\dag}$ be a matrix with singular values $\sn_1 \geq \sn_2 \geq
%\cdots \sn_n$ such that $\left\|N\right\|_F  < \frac{1}{100}\sigma_k$. Also, let $\calA(\cdot):\rmn \rightarrow \mathbb{R}^d$ be a linear measurement
%operator that satisfies $2k$-RIP with RIP constant $\delta_{2k}<\frac{(\sigma^*_k)^2}{100k(\sigma_1^*)^2}$.  Suppose, AltMin algorithm (Algorithm \ref{algo:sensing-altmin}) is supplied inputs $\aff$, $b=\aff(M+N)$. Then, after $T=4\log(2/\epsilon)$ steps, iterates $U^{T}$, $V^{T}$ of the AltMin algorithm  satisfy: 
%with $\dist\left(U^{(0)},U^*\right) \leq \frac{1}{2}$. Then $U^{(t)}$ and $V^{(t)}$ satisfy:
\begin{align*}
  \dist\left(\Vw^{T},V^*\right) \leq \frac{10\|N\|_F}{\so_k} + \epsilon, \ 
  \dist\left(\Uw^{T},U^*\right) \leq \frac{10\|N\|_F}{\so_k} + \epsilon.
\end{align*}
See Definition~\ref{defn:dist} for definition of $\dist\left(U, W\right)$. 
%where $\alpha_V, \alpha_U < 1$ are some constants depending only on $\delta_{2k}$. 
% denotes the principal angle based distance between subspaces spanned by the columns of $U\in \mathbb{R}^{m\times k}$ and $W\in \mathbb{R}^{m\times k}$ (See Definition~\ref{defn:dist}).
\end{theorem}
%\begin{theorem}\label{thm:sensing-noisy-main}
%   Let $M$ and $\calA(\cdot)$ be as defined in Theorem~\ref{thm:sensing_err}. 
%=U^*\Sigma^*V^{*^\dag }$ be a rank-$k$ matrix with non zero singular values $\sigma_1^*\geq \sigma_2^*\dots\geq \sigma_k^*$ and $N=\Un \Sn (\Vn)^{\dag}$ be the noise matrix. Also, let $\calA(\cdot):\rmn \rightarrow \mathbb{R}^d$ be a linear measurement operator that satisfies $2k$-RIP with RIP constant $\delta_{2k}<\frac{(\sigma^*_k)^2}{100k(\sigma_1^*)^2}$.  
%Suppose, \as algorithm (Algorithm \ref{algo:sensing-altmin}) is supplied inputs $\aff$, $b=\aff(M+N)$. Then, after $T=4\log(2/\epsilon)$ steps, iterates $\widehat{U}^{T}$, $\widehat{V}^{T}$ of \as  satisfy: 
%$$\|M-\widehat{U}\widehat{V}^T\|_F\leq C \|N\|_F,$$
%where $C=(\frac{\so_1}{\so_k}+10\delta_{2k})$. 
%\end{theorem}
At a high level, our proof for noisy case follows closely, the exact case proof given in Section~\ref{sec:sensing}. That is, we show that the update of \as algorithm is similar to power-method type update but with two errors terms: one due to incomplete measurements and another due to the noise matrix. A detailed proof of Theorem \ref{thm:sensing-noisycase} can be found in Appendix~\ref{app:noisy_sensing}.%One key difference is that top singular vectors of $M+N$ matrix are not exactly same as the singular vectors of $M$. Hence, we need to appropriately bound the distance of recovered matrices $\widehat{U}, \widehat{V}$ to the true singular vectors. 
%with $\dist\left(U^{(0)},U^*\right) \leq \frac{1}{2}$. Then $U^{(t)}$ and $V^{(t)}$ satisfy:
%\begin{align*}
%  \dist\left(V^{T},V^*\right) \leq \frac{10\|N\|_F}{\so_k} + \epsilon, \ \ \ 
%  \dist\left(U^{T},U^*\right) \leq \frac{10\|N\|_F}{\so_k} + \epsilon.
%\end{align*}
%See Definition~\ref{defn:dist} for definition of $\dist\left(U, W\right)$. 
%\end{theorem}
%The following theorem shows that if the Frobenius norm
%(sum of squared singular values) of the noise matrix $N$ is small enough, then alternating minimization gives a good approximation
%of $M$.
% We are now ready to prove Theorem \ref{thm:sensing-noisycase}.
% \begin{proof}(Theorem \ref{thm:sensing-noisycase})
%   From \eqref{eqn:sensing-orthogonaliter-error-noisycase}, \eqref{eqn:sensing-twonorm-noise-noisycase}, \eqref{eqn:sensing-twonorm-F},
% \eqref{eqn:sensing-twonorm-G-noisycase} and \eqref{eqn:sensing-minsingval-Rt-noisycase} we
% obtain the following:
% \begin{align*}
%   \dist\left(V^{(t)},V^*\right) = \twonorm{{V_{\perp}^*}^\dag V^{(t)}}
% 	&\leq \twonorm{{V_{\perp}^*}^\dag \left(Y \Lambda X^{\dag}U^{(t)}{R^{(t)}}^{-1} - {V_{\perp}^*}^\dag  F {R^{(t)}}^{-1} - {V_{\perp}^*}^\dag  G {R^{(t)}}^{-1}\right)} \\
% 	&\leq \twonorm{V_{\perp}^*}\left(\twonorm{Y \Lambda X^{\dag}U^{(t)}} + \twonorm{F} + \twonorm{G}\right)\twonorm{{R^{(t)}}^{-1}} \\
% 	&\leq 1 \cdot \left(\lambda_1 + \frac{\delta k \Gamma \dist\left(U^{(t)},U^*\right)}{1-\delta} + \frac{\delta \frob{\Lambda}}{1-\delta} \right) \cdot \frac{1}{\sigma_{\textrm{min}}\left(R^{(t)}\right)} \\
% 	&\leq \frac{ \lambda_1 + \frac{\delta k \Gamma \dist\left(U^{(t)},U^*\right)}{1-\delta} + \frac{\delta \frob{\Lambda}}{1-\delta} }
% 	{ \gamma \lambda - \lambda_1 - \frac{\delta k \Gamma \dist\left(U^{(t)},U^*\right)}{1-\delta} - \frac{\delta \frob{\Lambda}}{1-\delta} }.
% \end{align*}
% @@@complete this. The theorem follows from the above equation.
% \end{proof}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "altmin"
%%% End: 

